The Power of Constraint Grammars Revisited

Sequential Constraint Grammar (SCG) (Karlsson, 1990) and its extensions have lacked clear connections to formal language theory. The purpose of this article is to lay a foundation for these connections by simplifying the definition of strings processed by the grammar and by showing that Nonmonotonic SCG is undecidable and that derivations similar to the Generative Phonology exist. The current investigations propose resource bounds that restrict the generative power of SCG to a subset of context sensitive languages and present a strong finite-state condition for grammars as wholes. We show that a grammar is equivalent to a finite-state transducer if it is implemented with a Turing machine that runs in o(n log n) time. This condition opens new finite-state hypotheses and avenues for deeper analysis of SCG instances in the way inspired by Finite-State Phonology.

==> Makefile <==
all: 	
	xelatex graph
	bibtex  graph
	xelatex graph
	xelatex graph

allimg:  B-1.pdf B-2.pdf B-3.pdf B-4.pdf B-5.pdf B-6.pdf B-7.pdf B-8.pdf B-9.pdf B-6b.pdf B-1b.pdf B-2b.pdf B-V0.pdf B-T0.pdf B-VVV.pdf B-TTT.pdf B-VT.pdf B-TD.pdf
	@

B-%.pdf: B-%.dvi asr.tex
	dvipdf $<
	open $@

B-%.dvi: B-%.tex
	latex $<

dot-%.pdf: dot-%.dot2
	dot -Tpdf $< > $@
	open $@

dot-%.dot2: dot-%.dot
	perl -ne 's/->/€/go; s/\\n/ /go; s/label/arrowsize=.65,fontsize=10,label/go; s/node \[/node \[width=0.2,fontsize=10,/go; s/€/->/go; s/digraph A \{/digraph A \{  graph [fontname = "helvetica"]; node [fontname = "helvetica"]; edge [fontname = "courier"]; margin=0;rankdir = LR;ranksep=0;nodesep=.2; /; s/fontsize=10/fontsize=14/go; s/=filled/=solid/; s/@/NoTV/go; print;' < $<  > $<2 
#	perl -ne 's/->/€/go; s/>|<//go; s/label/arrowsize=.65,fontsize=10,label/go; s/node \[/node \[width=0.2,fontsize=5,label="",/go; s/€/->/go; s/digraph A \{/digraph A \{ margin=0;rankdir = LR;ranksep=0;nodesep=.2; node [width=0.2,style=invis,shape=circle,label=""] 00;/; s/\}/00 -> 0 [arrowsize=.65,fontsize=10];}/; s/=filled/=solid/; s/@/NoTV/go; print;' < $<  > $<2 

watt-%.natt: watt-%.att
	perl -ne 's/\@0\@/0/go; s/V/1/go; s/\[/2/go; s/\]/3/go; print' $< > $@

watt-%.sync: watt-%.att
	fstcompile -isymbols=syms -osymbols=syms $<  |\
	fstsynchronize | fstrmepsilon | fstprint -isymbols=syms -osymbols=syms > $@


